OpenStreetView-5M: The Many Roads to Global Visual Geolocation

Determining the location of an image anywhere on Earth is a complex visual task, which makes it particularly relevant for evaluating computer vision algorithms. Yet, the absence of standard, large-scale, open-access datasets with reliably localizable images has limited its potential. To address this issue, we introduce OpenStreetView-5M, a large-scale, open-access dataset comprising over 5.1 million geo-referenced street view images, covering 225 countries and territories. In contrast to existing benchmarks, we enforce a strict train/test separation, allowing us to evaluate the relevance of learned geographical features beyond mere memorization. To demonstrate the utility of our dataset, we conduct an extensive benchmark of various state-of-the-art image encoders, spatial representations, and training strategies. All associated codes and models can be found at https://github.com/gastruc/osv5m.

==> figures/dataset_bk2.tex <==
\pgfplotsset{%magma colormap
    /pgfplots/colormap={magma}{
        rgb255=(0,0,4)
        rgb255=(31,12,72)
        rgb255=(85,15,109)
        rgb255=(136,34,106)
        rgb255=(186,54,85)
        rgb255=(227,89,64)
        rgb255=(249,140,10)
        rgb255=(252,191,73)
        rgb255=(251,231,136)
        rgb255=(252,253,191)
    }
}

\begin{tabular}{c@{\;}c@{\;}c}

\begin{subfigure}{0.42\linewidth}
    \includegraphics[width=\linewidth]{images/density_train.png}
    \caption{Image density on the train set}
\end{subfigure}
&  %shared colormap with 2axis, nightmarish
\hspace{-1.8cm}
\begin{tikzpicture}
\node [draw=none] at (0,0) {
\begin{axis}[
    hide axis,
    scale only axis,
    height=3.7cm,
    width=0.5cm,
    colormap name=magma,
    colorbar,
    colorbar style={
        ymode=log,
        ymin=1, ymax=2500,
        ytick={1,10,100,1000},
        ytick pos=left,
        yticklabel pos=left,
        y axis line style={draw=none} % <-- Hides the y-axis line
    },
    point meta min=1, point meta max=2500,
    at={(2cm,0cm)} % Adjust position to place it next to the left y-axis
]
% This is the dummy plot:
\addplot [draw=none, forget plot] coordinates {(0,1) (1,1000)};
\end{axis}
};

\node [draw=none] at (1,0) {
\begin{axis}[
    hide axis,
    scale only axis,
    height=3.7cm,
    width=0.5cm,
    colormap name=magma,
    colorbar,
    colorbar style={
        ymode=log,
        ymin=1, ymax=150,
        ytick={1,10,100},
        ytick pos=right,      % <-- This ensures the y-ticks are on the right
        y axis line style={draw=none} % <-- Hides the y-axis line
    },
    point meta min=1, point meta max=150,
    at={(2cm,0cm)} % Adjust position to place it next to the left y-axis
]
% This is the dummy plot:
\addplot [draw=none, forget plot] coordinates {(0,1) (1,100)};
\end{axis}
};
\end{tikzpicture}
&
\begin{subfigure}{0.42\linewidth}
    \includegraphics[width=\linewidth]{images/density_test.png}
     \caption{Image density on the test set}
\end{subfigure}
\\

\multicolumn{3}{c}{
\begin{tabular}{c@{}c@{}c@{}c}
 \begin{subfigure}{0.24\linewidth}
 \includegraphics[width=\linewidth]{images/euro_train.pdf}
 \caption{Continent distribution in train}
 \end{subfigure}
 &
  \begin{subfigure}{0.24\linewidth}
 \includegraphics[width=\linewidth]{images/country_train.pdf}
  \caption{Country distribution in train}
 \end{subfigure}
 &
  \begin{subfigure}{0.24\linewidth}
 \includegraphics[width=\linewidth]{images/euro_test.pdf}
  \caption{Continent distribution in test}
 \end{subfigure}
 &
  \begin{subfigure}{0.24\linewidth}
 \includegraphics[width=\linewidth]{images/country_test.pdf}
  \caption{Country distribution in test}
 \end{subfigure}
\end{tabular}

}

\end{tabular}

==> figures/poster/dataset_poster.tex <==
\pgfplotsset{%magma colormap
    /pgfplots/colormap={magma}{
        rgb255=(0,0,4)
        rgb255=(31,12,72)
        rgb255=(85,15,109)
        rgb255=(136,34,106)
        rgb255=(186,54,85)
        rgb255=(227,89,64)
        rgb255=(249,140,10)
        rgb255=(252,191,73)
        rgb255=(251,231,136)
        rgb255=(252,253,191)
    }
}
\centering
\begin{tabular}{@{\hspace{-1mm}}c@{\;}c@{\;}c}
\begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{images/density_test2.png}
     \centering \scriptsize{Image density on test set}
\end{subfigure}
&  %shared colormap with 2axis, nightmarish
\hspace{-1.6cm}
\begin{tikzpicture}
\node [draw=none] at (0,-0.89) {};
\node [draw=none] at (0,0) {
\begin{axis}[
    hide axis,
    scale only axis,
    height=1.28cm,
    width=0.2cm,
    colormap name=magma,
    colorbar,
    colorbar style={
        ymode=log,
        ymin=0.000001, ymax=0.01,
        ytick={0.000001,0.0001,0.01},
        ytick pos=left,
        yticklabel pos=left,
        font=\tiny,
        %font=\fontsize{3pt}{3pt}\selectfont, % Extremely small font size
        y axis line style={draw=none}, % <-- Hides the y-axis line
    width=1*\pgfkeysvalueof{/pgfplots/parent axis width},
    },
    colorbar/width=5mm,
    point meta min=0.000001, point meta max=0.01,
    at={(2.0cm,0cm)} % Adjust position to place it next to the left y-axis
]
% This is the dummy plot:
\addplot [draw=none, forget plot] coordinates {(0,1) (1,1000)};
\end{axis}
};
\end{tikzpicture}

&
\begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{images/density_train.png}
     \centering\scriptsize{Image density on training set}
\end{subfigure}
\\

%\multicolumn{3}{c}{
%\begin{tabular}{c@{}c}
  \begin{subfigure}{0.40\linewidth}
   \begin{tabular}{c@{}c}
 \includegraphics[width=.45\linewidth]{images/euro_test.pdf}
 &
 \includegraphics[width=.44\linewidth]{images/country_test.pdf}
  \end{tabular}
  \centering \scriptsize{Distribution of test set}
 \end{subfigure}
 &
 &
\begin{subfigure}{0.40\linewidth}
 \begin{tabular}{c@{}c}
 \includegraphics[width=.45\linewidth]{images/euro_train.pdf}
 &
\includegraphics[width=.44\linewidth]{images/country_train.pdf}
 \end{tabular}
  \centering\scriptsize{Distribution of training set}
 \end{subfigure}
%\end{tabular}
%}
\end{tabular}

==> figures/spider_table.tex <==
\begin{table}[]
    \caption{{\bf Evaluation on other Datasets.}
    We use public evaluation datasets to compare the performance of our base and best models trained on OpenStreetView-5m as well as various geolocation approaches trained on other datasets. 
    $\dagger$ trained on non-public datasets.}
    \label{tab:registration}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}
        \toprule
        & \%@ & \%@ & \%@ & \%@ \\
        & 25km & 200km & 750km & 2500km \\
        \midrule
        Im2GPS \\\greyrule
        $\dagger$ StreetCLIP \cite{haas2023learning} &
        28.3 & 45.1 & 74.7 & 88.2 \\        
        Translocator \cite{translocator} & 48.1 & 64.6 & 75.6 & 86.7 \\
        Clark \cite{Google-World-Streets-15K-geolocation} & 50.2 & 69.0 & 80.0 & 89.1 \\
        base model 0.03 & 2.7 & 20.4 & 52.8 \\
        \midrule
        Im2GPS-3k \\\greyrule
        translocator \cite{translocator} & 31.1 & 46.7 & 58.9 & 80.1 \\
        StreetCLIP & 22.4 & 37.4 & 61.3 & 80.4 \\
        Clark \cite{Google-World-Streets-15K-geolocation} & 33.5 & 45.9 & 61.0 & 76.1 \\
        base model & 0.03 & 2.5 & 19.65 & 51.98 \\
        \midrule
        YFCC-4k \\\greyrule
        Clark \cite{Google-World-Streets-15K-geolocation} & 24.4 & 33.9 & 50.0 & 68.7\\
        translocator  \cite{translocator} & 18.6 & 27.0 & 41.1 & 60.4 \\
        base model 0.04 & 2.06 & 15.9 & 44.13 \\
        \midrule
        YFCC-26k \\\greyrule
        translocator & 17.8 & 28.0 & 41.3 & 60.6 \\
        Clark \cite{Google-World-Streets-15K-geolocation} & 23.9 & 34.1 & 49.6 & 69.0 \\
        base model \\
        \\
        \midrule
        GWS-15k \\\greyrule
        translocator & 1.1 & 8.0 & 25.5 & 48.3 \\
        Clark \cite{Google-World-Streets-15K-geolocation} & 1.5 & 8.7 & 26.9 & 50.5 \\
        base model \\
        best model \\
        \bottomrule
    \end{tabular}
    }
\end{table} 

==> graveyard.tex <==
\paragraph{Localizable \textit{v.s.} Non Localizable.} As with any cultural practice, taking images always involves and is associated with geographical information. From the pictured objects or human faces to the materials and the used camera sensor, all relate to actual or original geographies. However the fact that geographical information is linked to them, doesn't guarantee that it should be used as a signal to extract meaningful information from these images. For example, the image of a plate of cooked fish in a restaurant (see \figref{fig:data:geoloc}) taken in \TODO{LOIC ADD LOCATION - is it austria?} could have equivalently been taken in a restaurant in Argentina that pretends to be in \TODO{LOIC ADD LOCATION}. Indeed, we could estimate by analyzing the clothes of a person or the color of the sun being reflected in the plate, or by searching the name of the restaurant written on the plate, from which location it comes but such a detective work, seems to not be the primary focus of learning geographically informative features.

\color{Blue}
As with any computer vision task, we would like to be able to properly attribute progress among methods (architecture, losses) and datasets (scaling up, changing distribution). However, due to the lack of a standard, open, and large geolocation dataset, serving serving a role similar to ImageNet \cite{imagenet-1k} or LAION \cite{laion}, most approaches have to both tinker with the model and the architecture, making an "apples to apples" comparison, impossible.
The main reason for this, seems to be that there is no open large-scale available dataset specific to geolocation, and thus progress can only be measured according to a small collection of ever changing test benchmarks \cite{Im2gps, Google-World-Streets-15K-geolocation, YFCC-Val26k-Interpretable-semantic-photo-geolocation-DL}. Inspired by \cite{schmidt} we first group prior work according to scale (number of data points) and training distribution (how are the images collected and from which source).

\paragraph{Data} A major source of geolocation training data are crawled geotagged web photos. Early influential attempts, like Im2GPS \cite{Im2gps} and PlaNet \cite{PlaNet} crawled XM images from Flickr and 1M training images and 34M validation images \textit{randomly scraped and minimally filtered} from an unknown source. However, the source distribution of geotagged images was soon standardized through the release of YFCC100M \cite{yfcc100m} dataset. From this huge 100M Flickr image dataset, some geolocation specific splits have been proposed \cite{flickr-mouselly, split-yfcc} but the data is reported to be noisy and often ambiguous, even when curated \cite{Im2GPS++YFCC4k+Im2GPS3k, ISN, Google-World-Streets-15K-geolocation} and even geographically and often racially biased \cite{yfcc-analysis}. A more clean split of 14M images can be found in the not that commonly used \cite{flickr-mouselly}, half of which is in a proper resolution \cite{izbicki2020exploiting}. With all its limitations such a distribution ofters indeed a very challenging task, that certain approaches have solved in remarkable success \cite{Im2gps, Im2GPS++YFCC4k+Im2GPS3k, Google-World-Streets-15K-geolocation, izbicki2020exploiting}, however a more clean and realistic dataset, with images similar to those of Google Street View, seems like a missing contribution. Indeed the second most common data distribution is that of Google Street View (\textbf{GSV}) Images \cite{GoogleStreetView}, which is mostly noiseless, has great coverage properties and is captured with a fixed sensor. To the best of our knowledge the only available datasets of GSV images \cite{nn-UCF-GSV-Dataset-2014, mirowski2019streetlearn-navigation} provide 50K-100K densely sampled images from at most 3 major US cities (Pittsburgh, Orlando, Manhattan) with the intended application of place-recognition and street-navigation. However some succesful geolocation approaches have been trained on GSV images of the order of 100K \cite{luo2022geolocation} and 1M \cite{StreetCLIP}, but are limited in at mostly sharing panorama-ids due to copyright limitations\footnote{Official download of 150K images of \textit{non-shareable}, street-view images currently costs 1K \$ in Google Street View API credits.}. Even test sets, either when they come from YFCC \cite{Im2gps, Im2GPS++YFCC4k+Im2GPS3k, YFCC-Val26k-Interpretable-semantic-photo-geolocation-DL} or from GSV \cite{Google-World-Streets-15K-geolocation}, they come in significantly small quantities of the order of less than 30k images. To the best of our knowledge we provide the first large scale (5M train, 1M val) open dataset of GSV-like images. Note that on our datasource Mapillary \cite{apillary}, several datasets have been proposed for a plethora of tasks different from geolocation, including semantic segmentation \cite{map-vistas} (25K samples), lifelong place recognition (1.68M densely sampled trajectories from 30 cities) \cite{map-lifelong-pr}, visual localization ($<$2K) \cite{map-vloc}, traffic sign detection and classification \cite{map-traffic-signs}, and depth estimation (750K from 50k scenes) \cite{map-depth}.
The latter is the largest dataset that we could use for geolocation, but it comes in significantly less data (750K) in comparison to ours (5M) as well as coverage ().
We summarize all the above information that renders our dataset a contribution in Table~\ref{table:dataset-characteristics}.
}
\fi

==> templates/3DV/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> version_safe/1_intro.tex <==



%In contrast to image classification, where the focus is often a single object, the task of inferring geographical information from images often involves much more latent cognitive processes such as locating salient clues and synthesizing external information \cite{mehta2016exploratory}. In that way, w
While image classification is the dominant supervised task for evaluating computer vision methods \cite{imagenet-1k,ridnik2021imagenet,van2018inaturalist}, geolocation presents a compelling alternative, thanks to the abundance of available geotagged images and the difficulty of its objective. 
In contrast to image classification, where the focus is often a single object, robust global geolocation involves detecting 
various visual clues including road signage, architectural patterns, or climate and vegetation. These elements, acquired across diverse contexts and conditions, must then be combined and matched with a comprehensive understanding of the world's geography and cultures; see \figref{fig:teaser} for some examples.

Despite this potential, few supervised approaches have been trained and evaluated for the task of geolocation. We attribute this to the  limitations of existing geolocation datasets:
(i) Large and open geolocation datasets contain a significant portion of noisy and non-localizable images \cite{Im2gps,Im2GPS++YFCC4k+Im2GPS3k, izbicki2020exploiting};
(ii) Street View datasets are better suited for the task but are expensive and proprietary \cite{luo2022geolocation, StreetCLIP, Google-World-Streets-15K-geolocation,chen2011city,hausler2021patch,seymour2018semantically}. 
To address these issues, we introduce OpenStreetView-5M (OSV-5M), an open-access dataset of 5.45 million high-quality and crowd-sourced street view images. Our goal is to make global visual geolocation a new standard task for measuring the capacity of deep learning approaches. 

\begin{figure}
\definecolor{myred}{RGB}{255,0,0}
\definecolor{myMagenta}{RGB}{181,86,255}
\definecolor{mygreen}{RGB}{21,226,17}
\definecolor{myblue}{RGB}{10,5,255}
    \centering
    \begin{tikzpicture}
        \node (img) at (0,0) {\includegraphics[width=1\linewidth]{images/plonk_teaser.pdf}};
        \node[below right = -2mm and -60mm of img.south east, align=right] {\tiny drivephotograph, and\_eng, gclem, bootprint, Mapillary, licensed under CC-BY-SA.};
    \node[below=0mm of img.south] {
    \begin{tabular}{c}
    \begin{tabularx}{.9\linewidth}{cccc}
    \footnotesize               
    \hspace{-5mm}\textcolor{mygreen}{climate/vegetation} &
    \footnotesize  
    \textcolor{myred}{traffic markers} & 
    \footnotesize  
    \textcolor{myblue}{architecture}& 
    \footnotesize  
    \textcolor{myMagenta}{culture/script}
    \end{tabularx}
    \end{tabular}
    };
    \end{tikzpicture}  
    \vspace{-7mm}
    \caption{{\bf Visual Geolocation.} 
    Predicting the location of an image taken anywhere in the world just from pixels requires detecting a combination of clues of various abstraction levels \cite{mehta2016exploratory}. Can you guess where these images have been taken?\protect\footnotemark  }
    \label{fig:teaser}
\end{figure}

\footnotetext{
\rotatebox[origin=c]{180}
{
\begin{minipage}[t]{.96\linewidth}
From top left to bottom right: Nagoya, Japan; Ontario, Canada; Mato Grosso, Brazil; Lofoten, Norway.
 \end{minipage}
}
}

Automating visual geolocation has significant potential benefits, with direct applications in fields such as journalism, forensics, and even historical and cultural studies. Learning robust geographical representations may also be valuable for various deep learning applications such as image generation and the development of more interpretable AI systems.
Thanks to its size and scope,%, and a clean train/test split,
OSV-5M is a robust and reliable benchmark for computer vision models.
To demonstrate this, we provide extensive experiments demonstrating the impacts of various factors such as pre-training strategies, model scale, optimization methods, contrastive losses, and the role of auxiliary tasks.

==> version_safe/3_dataset.tex <==
\begin{figure}
\input{figures/geoloc}

\vspace{-1em}
\caption{{\bf Localizable vs Non-Localizable.}
Images from our dataset (green) occupy the space between weakly localizable (red) images like the ones from the test set of Im2GPS3k \cite{Im2GPS++YFCC4k+Im2GPS3k} and landmark images used to advertise CV conferences (blue).}
% Strongly localizable images offer clear visual cues for inferring or narrowing down location; (\ref{fig:data:geoloc:loc}) Weakly localizable images contain only indirect hints; (\ref{fig:data:geoloc:nonloc}) Non-localizable images lack apparent cues related to their location.}    
\label{fig:data:geoloc}
\end{figure}



In \secref{sec:data:localizability}, we start by defining the notion of image localizability.
We then present existing geolocation datasets in \secref{sec:related:data} and the main geolocation methods in \secref{sec:related:method}.

%introduce OpenStreetView-5M in \secref{sec:data:motivation} %We conclude this section by outlining the detailed dataset creation process in \secref{sec:data:constitution}.

%===============================================
\subsection{Localizability}
%==============================================
\label{sec:data:localizability}

As illustrated in \figref{fig:data:geoloc}, 
image localizability exists on a subjective spectrum \cite{izbicki2020exploiting}. Non-localizable images either lack information related to their location or are too low quality to analyze meaningfully. Weakly localizable images only contain vague or indirect hints; these often feature indoor scenes or focus on people, animals, or objects. Localizable images contain enough information to allow for an informed guess relative to their location. For example, street view images are generally localizable as they often capture salient features indicative of the local environment such as climate, architecture, or road marking. At the far end of the spectrum, landmark images showcase emblematic monuments or iconic landscapes, making them instantly identifiable to most observers.
Our visual inspection suggests that 35\% of the images in IMG2GPS3K, a dataset commonly used to benchmark geolocation methodologies \cite{Im2GPS++YFCC4k+Im2GPS3k}, are non-localizable.

\paragraph{Impact.} The presence of non-localizable images within a dataset can significantly compromise the reliability of model evaluations. Weakly localizable images may occasionally be pinpointed through painstaking investigation, such as identifying a restaurant's name or recognizing commercial brands; these efforts are tangential to the actual learning of geographical representations. Landmark images are made often trivially localizable by the landmark in question. Our dataset predominantly comprises street view images, which are typically localizable but whose accurate localization requires learning robust geographical image representations.

%======================================================
\subsection{Geolocation Datasets}
%=======================================================
\begin{table}[t]
     \centering
         \caption{{\bf Geolocation Datasets.} OpenStreetView-5M contains strongly localizable street views with access and size comparable to web-scraped databases.}
     \label{tab:dataset}
     \resizebox{\linewidth}{!}{
     \begin{tabular}{@{}llccc@{}}
          \toprule
         \multirow{2}{*}{Image Source} &\multirow{2}{*}{size} & open- & \multirow{2}{*}{scope}\\
         &&access&      \\\midrule
          Web-scrapped \\\greyrule
        Im2GPS \cite{Im2gps}  & 237 &\true & biased\\
         Im2GPS3k \cite{Im2GPS++YFCC4k+Im2GPS3k}  & 2997 &\true & biased\\
        YFCC4k \cite{Im2GPS++YFCC4k+Im2GPS3k}  & 4536 & \true & biased\\
        YFCC26k \cite{YFCC-Val26k-Interpretable-semantic-photo-geolocation-DL}  & 25,600 &\true & biased\\
        MP-16 \cite{split-yfcc} & 4.72M & \true & biased\\
        Moussely \etal \cite{flickr-mouselly} & 14M/6M \cite{izbicki2020exploiting} & \true & global \\
        YFCC100M \cite{yfcc100m}  & 100M & \true & biased \\
        PlaNet \cite{PlaNet}  & 125M & \false & biased \\
          \midrule
         StreetView \\\greyrule
        Google-WS-15k \cite{Google-World-Streets-15K-geolocation}  & 14,955 & \false & global \\
        GMCP \cite{nn-UCF-GSV-Dataset-2014} & 105K & \false & 3 cities \\
        StreetCLIP  \cite{StreetCLIP} & 1M & \false & unknown \\
          \bf OpenStreetView-5M & 5.45M &\true & global
         \\ \bottomrule
     \end{tabular}
    }

 \end{table}

\label{sec:related:data} 
We motivate the need for our dataset by reviewing the available geolocation datasets from the two current main sources of geotagged images: web-scraped and street view images. We present in \tabref{tab:dataset} a comparison between existing geolocation datasets and OpenStreetView-5M. 



\paragraph{Web-Scraped.}
Platforms like Flickr provide a near-endless source of geotagged images, such as the $100$ million images of YFC100M~\cite{yfcc100m}. 
These images have been captured by users and are often weakly or non-localizable,  featuring subjects like friends, pets, food, or art.
Furthermore, strongly localizable images typically focus on tourist spots, exhibiting a substantial cultural bias towards recognizable, often Western, landmarks \cite{yfcc-analysis}. The provided locations are occasionally missing or noisy, and the online nature of these images means they can be removed, hindering reproducibility
\footnote{60\% of the 2014 YFCC-split \cite{flickr-mouselly} had been deleted by 2020 \cite{izbicki2020exploiting}!}. For evaluation purposes, cleaner subsets have been proposed to improve both image distribution coverage and annotation quality \cite{YFCC-Val26k-Interpretable-semantic-photo-geolocation-DL,Im2GPS++YFCC4k+Im2GPS3k}. 
Despite their small scope and size, these datasets are currently the primary means of evaluating geolocation models
%These datasets are currently the primary means of evaluating geolocation models, though they are limited in scope and not subject to a strict split with the datasets used for training.


\paragraph{Street View.} 
Conversely, street view images tend to be strongly localizable. Captured through panoramic cameras or dash-cams, they display with high fidelity and clarity a vehicle's surroundings, which are mostly localizable outdoor scenes. Despite being the most common source of high-quality street view images, Google Street-View images are expensive to acquire for research use (\$1000 for 150K images) and non-shareable. Open datasets from this source either only consist of dense samples from 3 US cities meant for navigation \cite{mirowski2019streetlearn-navigation,nn-UCF-GSV-Dataset-2014}, or are inaccessible \cite{StreetCLIP,luo2022geolocation, Google-World-Streets-15K-geolocation}.

Luckily, crowd-sourced platforms such as Mapillary \cite{mapillary} offer a diverse and global array of open-access street view images for various environments, including dense cities, suburbs, or remote countryside. Images from this source have been used to construct several benchmarks for multiple tasks other than geolocation, including depth estimation \cite{map-depth}, semantic segmentation \cite{map-vistas}, traffic sign detection and classification \cite{map-traffic-signs}, place recognition \cite{map-lifelong-pr} and visual localization \cite{map-vloc}. Based on Mapillary images, OpenStreetView-5M is the first large-scale street view geolocation benchmark providing 5.45M open-access images with global coverage. OSV-5M has similar order of magnitude as YFCC-based geolocation train sets \cite{flickr-mouselly,split-yfcc} and comes with a clean test set that is 33 times bigger than the current largest Street view image test benchmark \cite{Google-World-Streets-15K-geolocation} (not openly accessible).

%====================================================
\subsection{Geolocation Methods}
%===================================================
\label{sec:related:method}
There is a rich literature on place recognition \cite{zhang2021visual} and visual localization \cite{sattler2018benchmarking,pion2020benchmarking,piasco2021improving,ding2019camnet,kendall2015posenet}, where the goal is to find the pose of images of a known scene. In contrast, visual geolocation predicts 2D coordinates on the globe and goes beyond matching specific content to include the ability to generalize to unseen areas \cite{hays2015large}.
Visual geolocation approaches can be categorized based on whether they treat geolocation as an image retrieval problem, a classification problem, or both.

\paragraph{Image Retrieval-Based Approaches.}
A straightforward method for image localization is to find a similar image 
in a reference dataset and predict its location.
The first successful approach involved retrieving the nearest image in a space of handcrafted features such as gist features \cite{oliva2006building}, textons \cite{martin2001database}, and color histograms \cite{Im2gps}. It was later improved with SIFT features and support vector machines  \cite{Im2gps-pp}.
The incorporation of deep features helped further enhance this approach \cite{Im2GPS++YFCC4k+Im2GPS3k}.
While these models typically have good performance given a significantly extensive and dense image database, they do not involve representation learning. Consequently, they may exhibit limited generalization to sparsely represented or dynamically changing environments.%, and are limited in their interpretability.

\paragraph{Classification-Based Approaches.}
Geolocation can be approached as a classification problem by discretizing latitude and longitude coordinates. The choice of partition is critical, ranging from regular grid cells \cite{PlaNet}, adaptive splits such as QuadTrees \cite{Google-World-Streets-15K-geolocation}, or semantic-driven \cite{ISPN}, combinatorial  \cite{CPlaNet}, administrative \cite{translocator,haas2023pigeon}, and hierarchical~\cite{Google-World-Streets-15K-geolocation,Im2GPS++YFCC4k+Im2GPS3k} partitions. 
Classification-based methods must strike a delicate balance between cell size and quantity; too few large cells limit performance, while numerous small cells makes the prediction difficult. Furthermore, a typical classification loss such as cross-entropy doesn't incorporate the spatial relationship between regions;
confusing two adjacent cells leads to the same penalty as getting the continent wrong.
% 


\paragraph{Hybrid Approaches.}
Matching and classification approaches can be combined to overcome the limitations of discretization. This can be achieved using ranking \cite{Im2GPS++YFCC4k+Im2GPS3k} or contrastive objectives \cite{efficientnet}. Haas et al. \cite{haas2023pigeon} utilize a classification and regression approach based on prototype networks. Finally, Izbicki et al. \cite{izbicki2020exploiting} go beyond single-location prediction by estimating probability distributions based on spherical Gaussians.

\begin{figure*}
\input{figures/dataset}
\vspace{-2mm}
    \caption{{\bf OpenStreetView-5M.} Proportions of images per country and continent for the train and test sets. We prioritize the uniformity of the test set's distribution across the globe, while the train set distribution is less uniform.}
\label{fig:data:dataset}
\end{figure*}

%\YAN{\paragraph{Methods} More diverse than the evolution of geolocation datasets, is that of methods. The first method for geolocation used 8-nearest-neighbors and 6-mode-mean-shift with statistical descriptors (like textons and color histograms or gist) \cite{Im2gps} and was later improved through a learning based methods (kernel-SVMs) stacked on top of SIFT-features \cite{Im2gps-pp}. PlaNet was the first approach to successfully improve on the problem by introducing deep-CNNs by treating it as a classification problem on a dense data-specific set of discrete cells. Although its improved performance was initially attributed to scaling, soon Im2GPS++ improved in performance with only 5\% of the original data through the use of both a classification and a retrieval loss \cite{Im2GPS++YFCC4k+Im2GPS3k}. Some follow-up works, focused on fixing the discretization problem, through combinatorial segment predictions or by a learnable (and more interpretable) mixture of Gaussians \cite{izbicki2020exploiting}. Other focused on providing interpretable solutions of hierarchical prediction and scene classification \cite{Google-World-Streets-15K-geolocation, ISN}, or scene-grounding \cite{ISPN, translocator} and guidebook grounding \cite{luo2022geolocation}. In parallel, contrastive learning methods were also shown to improve performance \cite{efficientnet, StreetCLIP}. Drawing from all these approaches we design a common architecture and training framework to ablate some of their component's importance in this dataset, as well and introduce a more interpretable performance score inspired by the game of geoguessr. Note that although in this work we don't discuss the neighboring tasks of place recognition \cite{NetVLAD} or cross-view geolocation \cite{HaysCrossView}, they may significantly benefit from our provided dataset.
%}

==> version_safe/4_benchmark.tex <==
We use OpenSteetView-5M as a benchmark for supervised deep-learning approaches in the context of visual geolocation. In \secref{sec:baseline}, we outline our versatile baseline mode. In later sections we explore several design choices, starting with the image encoder backbone in \secref{sec:backbone}, then with the prediction objective in \secref{sec:prediction}, the optimization strategy in \secref{sec:training}, as well as the contrastive losses in \secref{sec:contrast}. We conclude in \secref{sec:combined} with an analysis of the model combining all best-performing designs. 

\if 1 0
\begin{figure}
    \centering
    \includegraphics[width=\linewidth, height=.15\textheight]{images/geoscore.png}
    \caption{{\bf Geoscore.} From a point centered in Paris, red contours highlight level sets of the score along the earth's spherical geometry.}
    \label{fig:geoscore}
\end{figure}
\fi

\begin{table*}[]
    \caption{{\bf Impact of Image Encoder.} We evaluate several pretrained backbone methods on OpenStreetView-5M. In particular, we highlight the influence of various architectures, pre-training strategies, and datasets. 
    Best score in \textbf{bold}.
    We denote closed datasets with $\dagger$.}
    \label{tab:backbone}
    \centering
    \resizebox{.7\linewidth}{!}
    {\small
    \begin{tabular}{@{}llllccccccc@{}}
        \toprule
        archi-& size & \multicolumn{2}{c}{pre-training}& training & geo- & avg & \%@ & \%@ & \%@ & \%@ \\ \arrayrulecolor{black!30} \cline{3-4} \arrayrulecolor{black}
        tecture& $\times 10^6$ &strategy & dataset  & in h & score & dist $\downarrow$ &  country & region & area & city\\
        \midrule
       \textcolor{BASELINECOLOR}{ViT-B-32}& 88 & CLIP& LAION-400M & 22 & 2386 & 2464 & 41.0 & 9.1 & 0.6 & 0.3\\\greyrule
       ResNet50 & 23 & Classification & ImageNet-1k & 45 & 1489 & 4205 & 24.0 & 3.9 & 0.2 & 0.1\\
       ViT-L-14& 300 &  CLIP &  LAION-400M & 206 & 2820 & 1879 & 50.1 & 13.3 & 1.0 & 0.3\\
       ViT-L-14& 300 &  CLIP &  Meta-CLIP  & 206 & 3057 & 1480 & 55.0 & 15.6 & 1.3 & 0.4\\
       ViT-L-14& 300 & CLIP &  DATA\_COMP & 206 & 3073 & 1520 & 55.8 & 16.2 & 1.3 & 0.4\\
       ViT-L-14& 300 &  CLIP &  OpenAI$^\dagger$ & 206 & 3223 & 1294 & 58.8 & 17.9 & 1.5 & 0.5\\
       ViT-L-14& 300 &  StreetCLIP  &  OpenAI$^\dagger$ + GSV$^\dagger$ & 206 & \bf 3361 & \bf  1122 & \bf 62.0 & \bf 19.9 & \bf 1.8 & \bf 0.6\\
       ViT-L-14& 300& DINOv2 &  DINOv2$^\dagger$ & 316 & 2886 & 1742 & 52.8 & 13.3 & 0.9 & 0.3\\
       ViT-bigG-14& 1800 & CLIP & LAION-400M  & 900 & 3234 &  1333 & 58.9 & 18.5 & 1.7 & 0.5\\
   
        \bottomrule
    \end{tabular}
    }
\end{table*}

%==================================================
\subsection{Baseline Model}
%=================================================
\label{sec:baseline}
We denote the space of images by $\cI$ and the span of longitude and latitude coordinates by $\cC = [-180,180] \times [-90,90]$. Our objective is to design a model that maps an image from $\cI$ to its corresponding location in $\cC$.

%We use a simple baseline model described below to evaluate the influence of many different machine learning techniques in the context of geolocation.

\paragraph{Base Framework.}
All models considered in this paper consist of two modules:
(i) an image encoder $f^\text{img}:\cI \mapsto\bR^d$, which maps an image to a $d$-dimensional vector, and
(ii) a geolocator $f^\text{loc}:\bR^d \mapsto\cC$, which maps this vector to geographic coordinates.
Unless stated otherwise, $f^\text{img}$ is always a pretrained and frozen CLIP ViT-B/32 model \cite{Radford2021LearningTV} with $d=768$ and $f^\text{loc}$ is a Multilayer Perceptron (MLP) with GroupNorms \cite{wu2018group}. We directly regress geographical coordinates and uses the $L_1$ norm as a loss function. The resulting baseline model is denoted in \textcolor{BASELINECOLOR}{blue} and its performance serves as a reference to study the impact of various design choices. The model is trained with a batch size of $512$ images for $30$ epochs ($260$k iterations) with a fixed learning rate of $2\times 10^{-4}$.

\paragraph{Evaluation Metrics.}
We measure the performance across geolocation models with three distinct sets of metrics. First, we qualify the models' precision with the average Haversine distance \cite{van2012heavenly} between predicted and ground truth image locations. Then, we compute the rate at which the prediction falls within correct administrative boundaries, of increasing granularity: country, region, area, and city. Using administrative borders aligns better with actual applications than the standard per-km radius accuracy of Im2GPS \cite{Im2gps}.
%We find such a measure to be more informative than the standard per-km radius accuracy of Im2GPS \cite{Im2gps}, both because administrative borders have an influence in visual appearance and because it can suggest actual performance if used for actual applications.

The average distance metric is sensible to outliers and a few bad predictions can misrepresent the efficacy of a high performing algorithm. Conversely, the accuracy metric based on administrative borders may be too lenient for large divisions or arbitrarily restrictive for small ones. To circumvent these shortcomings, we also use the \textbf{Geoscore}, based on the famous Geoguessr game \cite{geoguessr}. Defined as $5000\exp(-\delta/1492.7)$~\cite{haas2023pigeon}, where $\delta$ denotes the error distance, this metric rewards appropriately precise predictions while not being overly sensitive to large but rare errors.
%=============================================
\subsection{Image Encoder}
%=============================================
\label{sec:backbone}
We experiment with various architectures for the image encoder backbone: ResNet50 \cite{he2016deep}, ViT-B-32, ViT-L-14, and ViT-biG-14 \cite{dosovitskiy2020image}. We also examine the impact of pretraining strategies: CLIP \cite{Radford2021LearningTV}, DINOv2 \cite{oquab2023dinov2}, and the geolocation-based StreetCLIP \cite{haas2023learning}.
We also evaluate the role of the datasets used to train image encoders. We considered both public datasets such as LAION-400M \cite{schuhmann2021laion}, DATA\_COMP \cite{datacomp}, Meta-CLIP \cite{xu2023demystifying}, as well as proprietary datasets at Google, FAIR, or OpenAI. We report the results of our experiments in \tabref{tab:backbone} and highlight several takeaways:
\begin{itemize}[itemsep=0em, wide, labelwidth=!, labelindent=2pt, topsep=0em, parsep=0em]
    \item \textbf{Model Size.} As expected, there appears to be a direct correlation between the size of the image encoder and its geolocation performance. For instance, upgrading the base CLIP-VIT-B-32 model with $88$M parameters to the larger L-14 variant with $300$M parameters results in a substantial boost of nearly $434$ geoscore points. The even larger bigG-14 model with $1.8$ billion parameters grants a further $414$ points.
    \item \textbf{Pretraining Dataset.} The choice of the pretraining dataset is also impactful. Whe considering the same ViT-L-14 architecture, shifting from LAION-400M to DATA-COMP leads to a geoscore improvement of $253$ points, while the proprietary OpenAI dataset brings $403$ points of improvement. The StreetCLIP model further improves this performance by $138$ points by fine-tuning on a closed Google Street View dataset. The best performing datasets being closed source, we cannot exclude contamination with the test set.
    \item \textbf{Pretraining Strategy.} Using DINOv2 for pretraining under-performs by $337$ points compared to its CLIP-OpenAI counterpart. As the pretraining datasets differ and are closed source, it is difficult to draw a robust conclusion. %\TODO{NICOLAS}
\end{itemize}
This experiment illustrates the potential of OpenStreetView-5M to evaluate the impact of various design choices for image encoders.

%=============================================
\subsection{Prediction Head}
%=============================================
\label{sec:prediction}

For the geolocator network $f^\text{loc}:  \bR^d \rightarrow \cC$, we examine a variety of architectures , tasks, and supervision schemes.

\paragraph{Regression.} $f^\text{loc}$ directly predicts coordinates in $\cC$ using an MLP (without activation for the last layer)supervised with the L$_1$ loss between true and predicted locations. To better handle the periodicity of the latitude, we also consider an approach where we predict the cosine and sine of the longitude and latitude and use trigonometric formulas to recover the coordinates \cite{mac2019presence}.

\paragraph{Classification.} The train set is divided into a set $\cK$ of $K$ divisions, such as countries or regions. 
We then define $f^\text{lookup}:\cK \mapsto \cC$, which associates each division to the average location of its training images. Meanwhile, $f^\text{classif}: \bR^d \mapsto \bR^K$ maps an image representation to the probability that the image was taken in each division. The predicted geolocation is then defined by the region with the highest probability: $f^\text{loc} = f^\text{lookup} \circ \argmax f^\text{classif}$. 
The function $f^\text{classif}$ is an MLP trained with cross-entropy, while$f^\text{lookup}$ is obtained directly from the training set.

We define the division set $\cK$ by using available administrative divisions: countries, regions, areas, and cities, that amount to $K=222$\text{, }$2.8$K\text{, }$9.3$K, and $69.8$K, respectively. We also use partitions adaptive to the density of training images: with a QuadTree of depth $10$ and maximum leaf size of $1000$, corresponding to $11$K cells.

\begin{table}[]
    \caption{{\bf Prediction Modules.} While classification methods perform better than regression---especially when using hierarchical objectives, hybrid regression-classification approach performs best. We \underline{underline} the accuracy for divisions that the method is specifically trained to categorize.
    }
    \label{tab:method:prediction}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}llcccccccc@{}}
        \toprule
       && num. of & geo- & avg & \%@ & \%@ & \%@ & \%@
      \\
      && classes &score & dist $\downarrow$ & country & region & area & city \\\midrule
      \multicolumn{2}{l}{ \textcolor{BASELINECOLOR}{Regression}} & \textbf{-} & 2386 & 2464 & 41.0 & 9.1 & 0.6 & 0.3\\
      &\multicolumn{1}{l}{sin/cos} & \textbf{-} & 1349 & 4587 & 15.0  & 2.7 & 0.2 & 0.0
      \\\greyrule
      \multirow{7}{*}{\rotatebox{90}{Classification}}\!\!\!&
      Country & 222 & 2537 & 2443 & \underline{63.8} & 6.9 & 0.4 & 0.1 \\
      & Region & 2.8k & 3073 & 2253 & {63.8} & \underline{38.5} & 3.1 & 0.9 \\
      & Area & 9.2k & 2402 & 3645 & 45.0 & 27.4 & \underline{14.6} &  6.7\\
      & City & 70k & 2.8 & 2582 & 59.0 & 35.9 & 11.9 & \underline{8.0} \\
      & Admin + hier. & 70K& 3278 & 2134 & \underline{65.8} & \underline{43.2} & \underline{15.7} & \bf \underline{9.7}\\
        \greycrule{2-9}
     & QuadTree &11k& 3140 & 2255 & 61.7 & 35.3 & 10.0 & 4.9\\
     & + hier. & 11k & {3281} & {2046} & 64.9 & 38.2 & 10.8 & 5.2 \\
      \greyrule
      \multicolumn{2}{l}{Hybrid} & 11K& \bf 3445 & \bf 1914 & \bf 68.4 & \bf 45.9 & \bf 15.9 &  9.3\\
      \bottomrule
    \end{tabular}
    }
\end{table}

\paragraph{Hierarchical Supervision.} We can exploit the nested nature of the administrative divisions and QuadTree cells to supervise all levels simultaneously \cite{Im2GPS++YFCC4k+Im2GPS3k}. We predict a probability vector \emph{at the finest resolution} (either city or maximum depth of the QuadTree), which we aggregate recursively to obtain predictions at all levels. We can now supervise with a cross-entropy term for each level. 

\paragraph{Hybrid Approaches.} Inspired by approaches in classification and retrieval \cite{haas2023pigeon,Im2GPS++YFCC4k+Im2GPS3k}, we combine regression and classification in a two-step approach for QuadTrees. We associate each cell $k$ in $\cK$ with its bounding box $b_k$ in $\cC^4$. We consider two functions: (i) $f^\text{classif} : \bR^d \rightarrow \bR^K$  similar to the classification approach, and (ii) $f^\text{relative}: \bR^d \rightarrow [-1,1]^{2K}$ outputs for each cell $k$ a pair of relative coordinates within the bounding box $b_k$, scaled such that $(0,0)$ points to the cell's average location and $[-1,1]^2$ spans the entire bounding box. We first select the division with the highest probability and predict a location from its bounding box with the predicted relative coordinates. During training, $f^\text{classif}$ is supervised with the cross-entropy, and $f^\text{relative}$ uses the $L_2$ loss between the predicted and true relative coordinate \emph{for the division that contains the true location}.

\paragraph{Analysis.} The performances of these strategies are reported in \tabref{tab:method:prediction}. Notable observations include:

\begin{itemize}[itemsep=0em, wide, labelwidth=!, labelindent=2pt, topsep=0em, parsep=0em]
    \item {\textbf{Regression.}} Predicting the sines and cosines does not help the regression model. We hypothesize that this is due to the high-gradient region of the trigonometric formula used.
    \item {\textbf{Classification.}} Classification methods generally perform well in geoscore and starkly improve their respective classification rates, \eg $+38.5\%$ region accuracy for the region classifier compared to the regression model. However, their influence on the average error distance is smaller. Coarse partitions, like countries, are limited by the low precision of $f^\text{lookup}$. Inversely, overly refined partitions such as cities lead to a more challenging classification setting with many labels. Quadtree-constructed labels achieve performance close to the administrative division-based classifier for all granularity, \eg $61.7\%$ \vs $63.8\%$ for country and $35.3\%$ \vs $38.5\%$ for regions. This compounds into an overall better performance, which shows that adapting the granularity of the label distribution according to the image density appears to be a successful heuristic. 
    \item \textbf{Hierarchical.} Supervising all granularity levels   simultaneously significantly improves the prediction, highlighting the underlying hierarchical nature of global geolocation.
    \item \textbf{Hybrid.} Hybrid methods bridge the gap between classification and regression, granting high precision without relying on overly fine-grained partitions.
\end{itemize}
Adaptive partitions, hierarchical supervision, and hybrid models significantly improve upon border-based partitions and direct regression. 
This experiment demonstrates the complexity of the task of global geolocation---a field which has received little attention in the literature.
%=============================================
\subsection{Optimization Strategies}
%=============================================

\begin{table}[]
    \caption{{\bf Optimization Strategies.} We compare the effect of unfreezing part or all of the image encoder.}
    \label{tab:method:training}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lcccccccc@{}}
        \toprule
        & train. & train. & geo- & avg &  \%@ & \%@ & \%@ & \%@ \\
        & par. \small $\times 10^6$& in h & score & dist $\downarrow$ &  country & region & area & city \\
        \midrule
        \textcolor{BASELINECOLOR}{Frozen} & 0.6 & 22 & 2386 & 2464 & 41.0 & 9.1 & 0.6 & 0.3\\\greyrule
        %LoRA-16 & 1.6 & 42 & 2488 & 2181 & 42.8 & 8.6 & 0.5 & 0.2\\
        LoRA-32 & 2.4 & 44 & 2416 & 2294 & 41.6 & 8.1 & 0.5 & 0.2\\
        Last block & 7.7 & 26 & 3100 & 1688 & 56.1 & 18.6 & 1.6 & 0.6\\
          \textcolor{FINETUNECOLOR}{Fine-tuning} & 88 & 132 & \bf 3286 & \bf 1570 & \bf 61.0 & \bf 23.6 & \bf 2.4 & \bf 1.0\\
        %scratch & 88 & -\\
        \bottomrule
    \end{tabular}
   }
\end{table}
\label{sec:training}
We evaluate various optimization schemes:% for training our model:
\begin{itemize}[itemsep=0em, wide, labelwidth=!, labelindent=2pt, topsep=0em, parsep=0em]
    \item \textbf{Frozen.} $f^\text{img}$ remains frozen, we only learn $f^\text{loc}$.
    \item \textbf{LoRA-32.} We fine-tune $f^\text{img}$ using the LoRA approach \cite{hu2021lora} with a bottleneck dimension of $32$.
    \item \textbf{Last block.} We unfreeze the last block of $f^\text{img}$, which is responsible for combining the token embeddings into a single image representation.
    \item \textbf{Fine-tuning.} We fine-tune $f^\text{img}$ from its pre-trained state.
    %\item \textbf{From Scratch.} We train $f^\text{img}$ from a random state.
\end{itemize}
%CLIP
\paragraph{Analysis.} In \tabref{tab:method:training}, we report the impact of these optimization strategies. Unfreezing the last transformer block leads to a larger improvement than LoRA while marginally increasing the training time. This suggests that the pretrained patch encoder can extract relevant token embeddings, while their combination needs to be significantly adapted to the geolocation task. 
Unfreezing the entire network leads to even better results when starting from a pre-trained state, at the cost of a substantially increased training time.
We denote this experiment in \textcolor{FINETUNECOLOR}{orange} and use it as a new reference model for the rest of the experiments. 

%However, training the network from a random initial state does not lead to comparable performance, suggesting that the supervisory signal of geolocation is too noisy and complex to train a network from scratch.



%=============================================
\subsection{Contrastive Objectives}
%=============================================


\label{sec:contrast}
Contrastive learning constructs positive and negative sample pairs from the training distribution and pushes representations of positive pairs close to each other while contrasting the negative ones \cite{chen2020simple,chopra2005learning}. Positive pairs can be formed within the same modality, such as diverse views of an object, or across different modalities, such as image-caption pairs. In the geolocation context, we propose two main approaches for constructing such pairs:


\begin{itemize}[itemsep=0em, wide, labelwidth=!, labelindent=2pt, topsep=0em, parsep=0em]
    \item \textbf{Geographic.} We match images if they are within the same administrative divisions: countries, regions, areas, cities, or QuadTree cell. We modify the dataloader to ensure each image is part of at least one positive pair. It is worth noting that an image can be involved in multiple positive pairs within the same batch.    


    \item \textbf{Text-Based.} Similar to Haas \etal \cite{haas2023learning}, we pair each image with a textual description of its location formed as the following string: ``An image of the city of \$CITY, in the area of \$AREA, in the region of \$REGION, in \$COUNTRY.''.
\end{itemize}

Contrarily to Haas \etal \cite{haas2023learning}, we use the MIL-NCE loss \cite{miech2020end} as our contrastive objective to account for the possibly multiple positive matches.%  We adopt the MIL-NCE loss \cite{miech2020end} as our contrastive objective, which extends the InfoNCE loss \cite{oord2018representation} to cases where each sample can have multiple positive matches.

\begin{table}[t]
    \caption{{\bf Contrastive Learning.} We report the performance of adding a contrastive objective to our model, defined by various notions of positive matches. }
    \label{tab:contrastive}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}llcccccc@{}}
        \toprule
        && geo- & avg & \%@ & \%@ & \%@ & \%@ \\
        && score & dist $\downarrow$ & country & region & area & city \\
        \midrule
        \multicolumn{2}{l}{\textcolor{FINETUNECOLOR}{none}} & 3286 & 1570 & 61.0 & 23.6 & 2.4 & 1.0\\\greyrule
        \multirow{5}{*}{\rotatebox{90}{geographic}} \!\!\!
        &country & 3268 & \bf 1501 & \bf 77.7 & 17.6 & 1.1 & 0.3\\
        &region & \bf 3506 &  1507 & 69.5 & \bf 43.3 & 4.3 & 1.1\\
        &area & 2898 & 2178 & 53.4 & 26.8 & \bf 6.4 & 1.6\\
        &city & 3449 & 1552 & 66.5 & 34.2 & 5.8 & \bf 1.9 \\
        &cell & 3431 & 1623 & 66.1 & 34.9 & 6.0 & 1.7\\\greyrule
        \multicolumn{2}{l}{text-based} & 3173 & 1661 & 72.6 & 16.5 & 1.1 & 0.3\\ 
        \bottomrule
    \end{tabular}
    }
\end{table} 

\if 1 0
\begin{align}
\sum_{i \in \mathcal{B}}
    \log\!\!\left(
    \frac{
        \displaystyle{\sum_{p \in \mathcal{P}_i}}
        \!
            e^{
            f^{\text{img}}(i)^\intercal 
            f^{\text{img}}(p)
            /T
            }
    }
    {
        \displaystyle{\!\sum_{p \in \mathcal{P}_i}}
        \!
            e^{
            f^\text{img}(i)^\intercal 
            f^\text{img}(p)/T
            }
            \!\!+\!\!\!\!\!\!
        \displaystyle{\sum_{n \in \mathcal{B} \setminus \mathcal{P}_i}}\!\!\!\!
            e^{
            f^\text{img}(i)^\intercal 
            f^\text{img}(n)
            /T
            }
    }
    \!\!\right),
\end{align}
with $\mathcal{P}_i \subset \mathcal{B}$ the set of image positively paired with $i$ and $T$ a temperature parameter set as $0.1$. If an image has only one positive match, this equation simplifies to the InfoNCE loss \cite{oord2018representation}.
\fi

\paragraph{Analysis.} In \tabref{tab:contrastive}, we report the performance of our different approaches for constructing contrastive pairs.  We observe a significant improvement in terms of performance, in particular when using regions to build positive pairs. This is consistent with regions being likely to present unique visual and cultural characteristics. This approach yields a much higher country and region classification rate compared to the classification-based approaches presented in Table \ref{tab:method:prediction}, suggesting that encouraging geographically consistent embeddings is advantageous for geolocation.

We also observe that using text as a proxy when geographically-consistent pairs exist is not beneficial.


\if 1 0
\begin{figure}
    \centering
    \includegraphics[width=\linewidth, height=.15\textheight]{example-image}
    \caption{{Contrastive Training.} Similarity heatmap for Ireland.}
    \label{fig:enter-label}
\end{figure}
\fi
\if 1 0
%=============================================
\subsection{Auxiliary Tasks}
%=============================================
\label{sec:auxiliary}
We predict the different auxiliary metadata presented in \secref{sec:data:motivation} with a dedicated MLP $f^\text{aux}: R^d \mapsto \bR^a$, where $a$ is the sum of the expected outputs dimension of the auxiliary tasks: $11$ land cover classes, $31$ climate types, 
$15$ soil types, $1$ binary prediction for the driving side, and $1$ value for the distance to the sea. All categorical variables are supervised with unweighted cross entropy terms, while the distance to the sea is supervised with the L1 norm.

\paragraph{Analysis.} The incorporation of auxiliary tasks encourage the model to focus on relevant geographical cues. In practice, we observe a modest impact; however, when combined, these auxiliary tasks contribute to an overall performance increase of approximately $+XX$ points.

\begin{table}[]
    \caption{{\bf Auxiliary Variables.} We report the impact on the geolocation performance of adding various auxiliary prediction classes. We also report the performance for each auxiliary variable as the overall accuracy on the test set and the number of classes in parenthesis. $\star$ regression task, evaluated with the NRMSE.}
    \label{tab:auxiliary}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lccccccc@{}}
        \toprule
        &perf & geo- & avg & \%@ & \%@ & \%@ & \%@ \\
        \% & score & dist $\downarrow$ & country & region & area & city \\
        \midrule
        no auxiliary & - & 3286 & 1570 & 61.0 & 23.6 & 2.4 & 1.0\\\greyrule
        land cover (11) & - & 3093 & 1723 & 56.8 & 19.6 & 1.7 & 0.7\\
        climate (31) & 54.4 & 3159 & 1652 & 57.6 & 21.2 & 2.0 & 0.7\\
        soil type (15) & 64.9 & 3234 & 1564 & 59.0 & 22.3 & 2.1 & 0.8\\
        driving side (1) & 95.9 & 3220 & 1577 & 59.8 & 22.1 & 2.1 & 0.8\\
        distance to sea ($\star$) & 461km & 3206 & 1585 & 57.5 & 22.0 & 2.0 & 0.8\\\greyrule
        all & - & 3273 & 1513 & 59.6 & 23.8 & 2.2 & 0.8\\\bottomrule
    \end{tabular}
    }
\end{table} 
\fi
%=============================================
\subsection{Combined Model}
%=============================================
\label{sec:combined}

Following our previous exploration and analysis, we assemble our most impactful design choices for each step into a strong geolocation baseline, denoted in \textcolor{COMBINEDCOLOR}{green}.
See \tabref{tab:final} for a quantitative performance comparison. With all our improvements, we observe a stark increase in the model's performance, with over $+1566$ of geoscore, an average distance more than halved, as well as significantly better classification rates at all levels of administrative divisions.
We also report the zero-shot performance of other pre-trained models on our test set. We cannot evaluate our models on other street view datasets as they are not open-access. 
\if 1 0
\begin{figure}
    \centering
    \includegraphics[width=\linewidth, height=.2\textheight]{example-image}
    \caption{{Attention Maps.} We visualize the attention queries of the last layer of the image encoder for the combined model. The model focuses on geographically relevant area are highlighted.}
    \label{fig:enter-label}
\end{figure}
\fi

\begin{table}[]
    \caption{{\bf Combined Model.} We report the improvements that result from combining our best performing design choices from each section in a single model.}
    \label{tab:final}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lcccccc@{}}
        \toprule
        & geo- & avg & \%@ & \%@ & \%@ & \%@ \\
        & score & dist $\downarrow$ & country & region & area & city \\
        \midrule
        {\tikzmark{base}~\textcolor{BASELINECOLOR}{Base model}} & 2386 & 2464 & 41.0 & 9.1 & 0.6 & 0.3\\\greyrule
        {\tikzmark{backbone}\;\;\;ViT-L-14 DC }& +687& -944 & +14.8 & +7.1 & +0.7 & +0.1 \\
       {\tikzmark{head}\;\;\;QuadTree} & +754 & -209 & +20.7 & +26.2 & +9.4 & +4.6 \\
       {\tikzmark{hybrid}\;\;\;\;\;Hybrid} & +305 & -341 & +6.7 & +10.6 & +5.9 & +4.4 \\    {\tikzmark{hierarchical}\;\;\;\;\;Hierarchical} & +141 & -209 & +3.2 & +2.9 & +0.8 & +0.3\\
        {\tikzmark{train}\;\;\;\textcolor{FINETUNECOLOR}{Fine-tuning}} & +900 & -894 & +20.0 & +14.5 & +1.8 & +0.7\\
    {\tikzmark{contrast}\;\;\;\;\;Region contrastive} & +220 & -63 & +8.5 & +19.7 & +1.9 & +0.1
       \\\greyrule
        \multirow{2}{*}{\textcolor{COMBINEDCOLOR}{Combined model}} & +1566 & -1273 & +36.2 & +43.3 & +18.3 & +10.3\\
        & 3852 & 1191 & 77.2 & 52.3 & 18.9 & 10.6\\
        \greyrule
        %Random & 404 & 7998 & 5.0 & 0.2 & 0.0 & 0.0 \\
        {GeoEstimator \cite{muller2018geolocation}} & 1694 & 4765 & 30.7 & 8.7 & 3.2 & 1.4 \\
        {StreetCLIP (0-shot) \cite{StreetCLIP}} & 2450 & 2808 & 41.0 & 22.9 & 10.5 & 15.1 \\
        \bottomrule
    \end{tabular}
    \begin{tikzpicture}[overlay,remember picture]
    \draw[black,thick] ([yshift=1mm]pic cs:base) -- ([yshift=1mm]pic cs:backbone) -- ([xshift=2.5mm,yshift=1mm]pic cs:backbone) ;
    \draw[black,thick] ([yshift=1mm]pic cs:backbone) -- ([yshift=1mm]pic cs:head) -- ([xshift=2.5mm,yshift=1mm]pic cs:head) ;
    \draw[black,thick] ([xshift=1.25mm,yshift=1mm]pic cs:head) -- ([xshift=1.25mm,yshift=1mm]pic cs:hybrid) -- ([xshift=4mm,yshift=1mm]pic cs:hybrid) ;
    \draw[black,thick] ([xshift=1.25mm,yshift=1mm]pic cs:hybrid) -- ([xshift=1.25mm,yshift=1mm]pic cs:hierarchical) -- ([xshift=4mm,yshift=1mm]pic cs:hierarchical) ;
    \draw[black,thick] ([yshift=1mm]pic cs:head) -- ([yshift=1mm]pic cs:train) -- ([xshift=2.5mm,yshift=1mm]pic cs:train) ;
    \draw[black,thick] ([xshift=1.25mm,yshift=1mm]pic cs:train) -- ([xshift=1.25mm,yshift=1mm]pic cs:contrast) -- ([xshift=4mm,yshift=1mm]pic cs:contrast) ;
\end{tikzpicture}
    }
\end{table} 

 \paragraph{Nearest Neighbor (Retrieval).} We use the image encoder to perform retrieval by matching each image from the test set with an image from the train set based on the cosine distance between the image encoder's features.
 We perform approximate matching with the FAISS algorithm \cite{faiss} through the autofaiss package \cite{autofaiss}.  Performing retrieval with our baseline model for the entire test set takes $7$ hours and requires $19.1$~GB of cumulative storage. In comparison, the inference time of our combined model is $180$~min and its size is $1.2$~GB.

As reported in Table~\ref{tab:final_nn}, retrieval methods trained through contrastive learning exhibit high performance. However, the supervision of our combined model based on geographic coordinates and cells does not enhance its retrieval performance. In fact, its retrieval score is lower than its pretrained image encoder, and even below its performance when directly predicting geographic coordinates. These findings underscore the challenges inherent in training models for retrieval tasks.

 \begin{figure}[t]
    \centering
    \input{figures/aux}
    \vspace{-3mm}
    \caption{{\bf Auxiliary Supervision.} We report the performance with and without auxiliary supervision for training sets of different sizes. }
    \label{fig:aux}
\end{figure}
\begin{table}[]
    \caption{{\bf Nearest Neighbors.} We report the performance of nearest neighbors methods using different encoders.}
    \label{tab:final_nn}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lcccccc@{}}
        \toprule
        & geo- & avg & \%@ & \%@ & \%@ & \%@ \\
        & score & dist $\downarrow$ & country & region & area & city \\
        \midrule
        CLIP-VIT-B32-LAION & 2852 & 2855 & 55.2 & 35.6 & 23.5 & 17.3 \\
        CLIP-VIT-B32-OpenAI & 2983 & 2582 & 57.9 & 37.3 & 24.7 & 18.0 \\
        DINOv2 & 3387 & 1923 & 68.3 & 45.3 & 31.0 & 22.8 \\
        CLIP-VIT-L14-DATACOMP & 3570 & 1529 & 71.0 & 46.5 & 31.4 & 22.8 \\
        CLIP-VIT-L14-OpenAI & 3903 & 1029 & 78.7 & 53.8 & 37.1 & 26.7 \\
        StreetCLIP & \bf 3951 & \bf 974 & \bf 79.5 & \bf 55.2 & \bf 38.4 & \bf 27.7  \\ \greyrule
        %MBase model \\
%         Accuracy:  (country), 53.75 (region), 37.12 (sub-region), 26.70 (city)
% Haversine: 1028.88 (haversine),  (geoguessr)
        \textcolor{COMBINEDCOLOR}{Combined  model} &3108& 2055 & 61.3 & 32.2 & 18.8 & 13.0\\
        \bottomrule
    \end{tabular}
    }
\end{table} 
 

\paragraph{Error Distribution.}
We report in \figref{fig:final:distribution} a heatmap of the average error distance across the map. Areas sparsely populated with training images, such as South America, have a significantly higher error rate. We report a Pearson correlation coefficient of $-0.25$ between image density and error, suggesting that image density is not the only factor in the mistakes of our proposed model. See \figref{fig:final} for a visualization of the error distribution.

\paragraph{Auxiliary Variables.} We use an MLP $f^\text{aux}$ to predict the image's metadata in addition to its coordinates. As reported in \figref{fig:aux}, auxiliary supervision helps for smaller training sets. However, with enough data, our model learns powerful latent variables and does benefit from auxiliary supervision. %We provide further details on this negative outcome in the Appendix.



\paragraph{Annotator Performance.} We asked $80$ annotators to guess the locations of the same $50$ images randomly sampled from the test set \cite{mehta2016exploratory}, see following \href{https://huggingface.co/spaces/osv5m/plonk}{link}. The results are reported in \tabref{tab:humans}, and are compared with our models as well as two random baselines: selecting a random point on the map, and choosing the location of a random image from the training set. We also construct an Annotator Ensemble Oracle by selecting the most accurate prediction for each image from all annotators. Despite the inherent difficulty of the task, annotator performance is significantly better than chance. Our baseline model, and more substantially our combined model, surpasses the accuracy of individual annotator, but is still outmatched by the Annotator Ensemble Oracle.



\begin{figure}
    \centering
    \include{./figures/errormap}
    \caption{{\bf Error Distribution.} We plot the average prediction error of the combined model in km. %We observe a normalized correlation between image density and prediction error of $44\%$.
    }
    \label{fig:final:distribution}
\end{figure}


\begin{table}[]
    \caption{{\bf Annotator Performance.} We report the  performance of $80$ annotators on a subset of 50 images.}
    \label{tab:humans}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lccccc@{}}
        \toprule
        & geo- & avg & \%@ & \%@ & \%@\\
        & score & dist $\downarrow$ & continent & country & region\\\midrule
        Annotator performance & 1009 & 6407 & 48.9 & 12.2 & 3.0\\
        Annotator ensemble oracle & 3919 & 443 & 98.0 & 70.0 & 28.0\\ \greyrule
        Random location & 120  & 10273   & 16.0 & 0.0 & 0.0\\
        Random image & 328   & 8724 & 20.0 & 2.0 & 0.0 \\\greyrule
        Base model & 2317 & 2849 & 74.0 & 38.0 & 8.0\\
        \textcolor{COMBINEDCOLOR}{Combined model} & 3655 & 1516 & 88.0 & 72.0 & 46.0\\\bottomrule
    \end{tabular}
    }
\end{table} 

\begin{figure}

\pgfplotstableread[col sep=comma]{./data/histogram_baseline.csv}\datatablebaseline
\pgfplotstablecreatecol[
    create col/expr={
        \pgfmathaccuma + \thisrow{density}
    }
]{cumulative}{\datatablebaseline}

\pgfplotstableread[col sep=comma]{./data/histogram_random.csv}\datatablerandom
\pgfplotstablecreatecol[
    create col/expr={
        \pgfmathaccuma + \thisrow{density}
    }
]{cumulative}{\datatablerandom}
   
\pgfplotstableread[col sep=comma]{./data/histogram_humans.csv}\datatablehumans
\pgfplotstablecreatecol[
    create col/expr={
        \pgfmathaccuma + \thisrow{density}
    }
]{cumulative}{\datatablehumans}   

\pgfplotstableread[col sep=comma]{./data/histogram_combined.csv}\datatablecombined
\pgfplotstablecreatecol[
    create col/expr={
        \pgfmathaccuma + \thisrow{density}
    }
]{cumulative}{\datatablecombined}   

\pgfplotstableread[col sep=comma]{./data/histogram_streetclip.csv}\datatablestreetclip
\pgfplotstablecreatecol[
    create col/expr={
        \pgfmathaccuma + \thisrow{density}
    }
]{cumulative}{\datatablestreetclip}   

    \centering
    \begin{tikzpicture}
    \begin{axis}[
    ymode=log, % log scale for the y-axis
    %xlabel={Proportion of the Dataset},
    ylabel={Distance (km)},
    legend style={at={(1,-0.15)}},
    legend columns=3, 
    ytick={25, 200, 750, 2500, 7000, 20000}, % Specified y-ticks
    yticklabels={25km, 200km, 750km,  2500km, 7000km, 20000km}, % Custom y-tick labels
    xtick={0, 0.25, 0.5, 0.75, 1}, % Specified x-ticks
    xticklabels={0\%, 25\%, 50\%, 75\%, 100\%}, % Custom x-tick labels
    xmin=0, xmax=1, % x-axis limits
    ymin=5, ymax = 23000, % y-axis minimum
    enlargelimits=0.00,
    ymajorgrids=true, % to add major grid lines on the y-axis
    grid style=dashed,
    yticklabel style={
        font=\scriptsize,
        xshift=6.8cm
    },
    height=5cm,
    width=\linewidth
]

\addplot [no markers, red, very thick, dashed] table[x=cumulative, y=bin] {\datatablerandom};

\addplot [no markers, blue, very thick, dashed] table[x=cumulative, y=bin] {\datatablehumans};

\addplot [no markers, magenta, very thick, dotted] table[x=cumulative, y=bin] {\datatablestreetclip};

\addplot [no markers, BASELINECOLOR, very thick] table[x=cumulative, y=bin] {\datatablebaseline};

\addplot [no markers, COMBINEDCOLOR, very thick] table[x=cumulative, y=bin] {\datatablecombined};

\addplot [no markers, COMBINEDCOLOR, very thick, dotted] table[x=cumulative, y=bin] {\datatablecombined};

\legend{\scriptsize Random, \scriptsize Annotators$^\star$,\scriptsize StreetCLIP retr., \scriptsize Baseline,\scriptsize Combined,\scriptsize Combined retr.}

\end{axis}
\end{tikzpicture}
    \caption{{\bf Distribution of Error.} Proportion of predictions within a set distance in the test set. $^\star$ evaluated on $50$ images only.  \vspace{-2mm}}
    \label{fig:final}
\end{figure}
\if 1 0

\begin{figure}
    \centering
    \input{figures/spider}
    \caption{{\bf Evaluation on other Datasets.} We evaluate our base and best models on 5 public geolocalization benchmarks. We report the proportion of predictions within 25km, 200km, 750km, and 2000km of the true image position.}
    \label{fig:spider}
\end{figure}
\fi
